Statistical process discovery

Stochastic process discovery is concerned with deriving a model capable of reproducing the stochastic character of observed executions of a given process, stored in a log. This leads to an optimisation problem in which the model's parameter space is searched for, driven by the resemblance between the log's and the model's stochastic languages. The bottleneck of such optimisation problem lay in the determination of the model's stochastic language which existing approaches deal with through, hardly scalable, exact computation approaches. In this paper we introduce a novel framework in which we combine a simulation-based Bayesian parameter inference scheme, used to search for the ``optimal'' instance of a stochastic model, with an expressive statistical model checking engine, used (during inference) to approximate the language of the considered model's instance. Because of its simulation-based nature, the payoff is that, the runtime for discovering of the optimal instance of a model can be easily traded in for accuracy, hence allowing to treat large models which would result in a prohibitive runtime with non-simulation based alternatives. We validate our approach on several popular event logs concerning real-life systems.

==> pic_latex/table1.tex <==
\begin{table}[ht]
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l p{1ex} l p{1ex} l l l l l p{1ex} l l l}
        \toprule 
        Event log & & \#tr & & \multicolumn{5}{l}{ABC-SMC} & & \multicolumn{3}{l}{Best estimator} \\
        \cmidrule(){5-9} \cmidrule(){11-13}
         & & & & $M$ & $N$ & $(\epsilon_i)_{1 \leq i\ \leq M}$ & rEMD &  runtime & & name & rEMD &  runtime\\
        \hline
        BPIC13\_c & & 19 & & $5$ & $100$ & $[0.6 \xrightarrow{0.1} 0.2]$ & $0.13$ & $643s$ & & fork & $0.63$ & $0.007s$ \\
        BPIC13\_o & & 20 & & $5$ & $100$ & $[0.6 \xrightarrow{0.1} 0.2]$ & $0.16$ & $2402s$ & & pairs & $0.24$ & $0.003s$ \\
        BPIC17\_ol & & 11 & & $3$ & $100$ & $[0.2 \xrightarrow{0.05} 0.1]$ & $0.09$ & $848s$ & & freq & $0.09$ & \num{6.7e-5}$s$ \\
         & & & & $3$ & $500$ & $[0.2 \xrightarrow{0.05} 0.1]$ & $0.05$ & $3950s$ & & freq & $0.09$ & \num{6.7e-5}$s$ \\
        BPIC20\_dd & & 43 & & $10$ & $100$ & $[0.98 \xrightarrow{0.02} 0.8]$ & $0.67$ & $827s$ & & fork & $0.93$ & $0.009s$ \\
         & & & & $13$ & $100$ & $[0.98 \xrightarrow{0.02} 0.65]$ & $0.62$ & $1126s$ & & fork & $0.93$ & $0.009s$ \\
        BPIC20\_rfp & & 51 & & $13$ & $100$ & $[0.98 \xrightarrow{0.02} 0.8 \xrightarrow{0.05} 0.65]$ & $0.62$ & $2121s$ & & freq & $0.99$ & $0.002s$\\
        Roadfines & & 34 & & $7$ & $100$ & $[0.4 \xrightarrow{0.05} 0.1]$ & $0.2$ & $11284s$ & & pairs & $0.27$ & $0.017s$ \\
        \bottomrule
    \end{tabular}
    }
    \caption{Comparing ABC-SMC weight estimation on real-life logs.}
    \label{tab:exp1}
\end{table}

==> pic_latex/table2.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l p{1ex} c c p{1ex} c c p{1ex} c c}
        \toprule 
        Event log & & \multicolumn{2}{l}{log properties} & & \multicolumn{2}{l}{net properties} & & \multicolumn{2}{l}{reachability graph}\\
        \cmidrule(){3-4} \cmidrule(){6-7} \cmidrule(){9-10}
         & & \#dpi & \#at & & \#pl & \#tr & & \#state & \#tr \\
        \hline
        BPIC13\_c & & 183 & 4 & & 16 & 19 & & 46 & 176 \\
        BPIC13\_i & & 1511 & 4 & & 17 & 23 & & 90 & 352 \\
        BPIC13\_o & & 108 & 3 & & 16 & 20 & & 74 & 264 \\ 
        BPIC17\_ol & & 16 & 8 & & 6 & 11 & & 6 & 11 \\
        BPIC20\_dd & & 99 & 17 & & 26 & 43 & & 235 & 1147 \\
        BPIC20\_rfp & & 89 & 19 & & 33 & 51 & & 247 & 1292 \\
        Roadfines & & 231 & 11 & & 29 & 34 & & 906 & 6526 \\
        \bottomrule
    \end{tabular}
    \caption{Event logs, nets and reachability graphs statistics.}
    \label{tab:prop}
\end{table}


==> sections/introOld.tex <==
\section{Introduction}
\section{Introduction}
\label{sec:intro}
%Process mining~\cite{10.5555/2948762}, inductive miner~\cite{DBLP:conf/apn/LeemansFA13}, alpha~\cite{1316839}, heursitic~\cite{tonbeta166}, linear programming~\cite{10.1007/978-3-540-68746-7_24}, fodina~\cite{VANDENBROUCKE2017109}, split~\cite{10.1007/s10115-018-1214-x}

A \emph{business process} consists in a set of activities performed so to accomplish a specific organisational goal. 
Understanding business processes is of prime importance for organisations in many respects: firstly, to obtain a formal description of often undocumented processes, then to use the obtained \emph{process model} to monitor and possibly improve the process under study. 
The principle goal of \emph{process mining}~\cite{10.5555/2948762}  is to   \emph{discover} a process model by exploiting the data that information systems of organisations accumulate in the form of \emph{event logs}. An event log consists of a collection of traces where each \emph{trace} is formed by a sequence of timestamped activities representing one observed case of the process. Since the same sequence of actions may be observed in multiple cases of a process, the same event log may contain multiple occurrences of the same trace, therefore leading to  \emph{trace frequency} being inherently associated with traces of a log: trace frequency quantifies how many times each unique sequence of actions has been observed, hence how likely it is the process exhibits the corresponding behavior.

\emph{Process discovery} algorithms~\cite{DBLP:conf/apn/LeemansFA13,1316839,tonbeta166,10.1007/978-3-540-68746-7_24,VANDENBROUCKE2017109,10.1007/s10115-018-1214-x} analyse an event log in order to \emph{mine} a formal model, commonly a Petri net,  aimed at capturing the \emph{control-flow}  of the observed process and hence reproducing the \emph{log language}, that is: the \emph{model language}, issued by the model's operational semantics, should be close to the log language. 
% given by the sequence of events that can occur in the model, should be close to  the log language. 
Evaluating the resemblance between a mined model and its corresponding log is the subject of \emph{conformance checking} analysis, which includes criteria such as assessing how many traces of the log are reproduced by the model  (\emph{fitness}) and conversely, how many traces of the model are not amongst that of the log (\emph{precision}). Certain mining algorithms, e.g., inductive miner~\cite{DBLP:conf/apn/LeemansFA13}, guarantee, by construction,  that the mined model fits the log.
%\plg{PLG: Here, "fits" has to be understood up the notion of model fitness ?}\pb{Yes precisely}
%Process mining approaches have proven fundamental  to improve business process management and have  attracted the interest of a wide research community. Nevertheless `standard'' \emph{discovery} approaches  are affected by an inherent weakness as they do not consider a very valuable source of information contained in the logs, that is,  trace frequency. This may  severely undermine the ability to take business analysis 

Although proven effective in many respects, "standard" \emph{discovery} approaches are affected by an inherent weakness as they do not consider a very valuable source of information contained in the logs, that is,  trace frequency. This may severely undermine the ability to improve the modelled business as the discovered models cannot reproduce the likelihood of the observed behaviours.  That leads to \emph{stochastic process mining} whose goal is discovering stochastic models which, other than the control flow also reproduce the likelihood of the observed process. 
This can be achieved either \emph{indirectly}, i.e., using a standard miner to obtain a control flow model and then, based on the trace frequencies, devising adequate \emph{weights} to convert it into a stochastic model~\cite{DBLP:conf/icpm/BurkeLW20}, or \emph{directly}, i.e., by devising a stochastic model straight from the log~\cite{DBLP:conf/apn/BurkeLW21}. 
In the stochastic settings, the resemblance between models and logs (i.e.,  \emph{stochastic conformance checking}) concerns the resemblance between \emph{stochastic languages}.  The most popular Earth Movers Stochastic Conformance (EMSC) measure~\cite{10.1007/978-3-030-26643-1_8,LEEMANS2021101724} is obtained as an adaptation of the Earth Movers Distance (EMD or Wasserstein distance) to the stochastic languages case. 

%However, it requires truncation when dealing with languages containing infinite words (a typical situation with models comprising loops).  
%suffers from implementation issues when it comes with dealing with  languages containing infinite words (a typical situations with models comprising loops).  Alternatively stochastic conformance can be assessed through  \emph{entropy} measures~\cite{Polyvyanyy2020AnER,Leemans:955905} which, differently from EMD, do not require truncation  in order to deal with infinite words. 
%An alternative to EMD  is  that of \emph{entropy} related conformance~\cite{Polyvyanyy2020AnER} Most recent developments~\cite{Leemans:955905} introduced novel entropy related conformance measures based on translation of both the log and the mined model into stochastic deterministic finite automata. 


%which, similarly to  Burke \emph{et al}'s~\cite{DBLP:conf/icpm/BurkeLW20}, is based on  \emph{weight estimation}, that is: we aim at estimating the \emph{weight} parameters for the transitions of a mined workflow Petri net in order to turn it into a stochastic Petri net which stochastically conforms the event log. %whose stochastic language resemble that of the event log. 
%To this aim, Burke \emph{et al}. introduced a few weight estimators, which combine simple statistics computed on the log with statistics computed on the model based on structural relationships of the Petri net's nodes. 
%To this aim Burke \emph{et al}.  introduced six kinds of weight estimator, which combine summary statistics computed on the log (e.g.  number of times  a subsequence of activities  is present in the log's  traces) with  structural relationships between the Petri net's nodes (e.g.  \emph{transitions causality}). %some consisting of simple  statistics computed  exclusively on the log's traces, other that combine log's trace statistics with  structural relationships between the Petri net's nodes (places and transitions). 
%Burke's estimators enjoy being computationally light, as, by definition, they do not need assessing the language of the Petri net model. However, the price for such simplicity is paid in terms of conformance as the distance between the resulting model's and the log's stochastic languages appears, in many cases, to be far from optimal. 

In this paper we consider the indirect stochastic process discovery approach and
propose a framework based on numerical optimisation to obtain optimal weights for the transitions of the Petri net. Our approach relies on calculating the probability that a given trace is produced by a stochastic Petri net as function of its transition weights. We do so by the construction of a dedicated \emph{unfold directed acyclic graph} whose nodes store the probability of finite prefixes as they are unfolded from the Petri net's reachability graph. 
Then, in order to optimize the weights, we need to measure the distance between the stochastic language of the event log and that of the Petri net.  We consider two distance measures, the Kullback-Leibler divergence and the earth moving distance.
Minimizing the Kullback-Leibler divergence corresponds to the maximum likelihood principle and leads to an efficient way to measure the divergence between the event log and the Petri net model. The earth moving distance is more popular in the area of stochastic languages but requires considerably more computational effort. To the best of our knowledge divergence based numerical weight optimization has not been experimented with before.

The paper is organised as follows: in Section~\ref{sec:prelim} we introduce preliminary notions the remainder of the manuscript relies upon; in Section~\ref{sec:method}, we describe the novel stochastic discovery approach we propose whereas in Section~\ref{sec:results} we demonstrate its application through a number of experiments on popular real-life event logs. We wrap up the manuscript with conclusive remarks and future perspectives in Section~\ref{sec:conclusion}.

%\medskip
%\noindent
%\pb{add reference to Conformance checking literature ?}\\
%\pb{certainly add reference to entropy based stochastic Conformance checking literature }\\
%\pb{add reference to Rogge-Stolte method: in the Related work subsection?}

\subsection{Related work}
To the best of our knowledge combination of statistical model checking and  process mining is a fairly novel research line with, so far,  very few contributions.  In~\cite{fi15120378} authors proposed a framework where SMC is pipelined to stochastic process discovery and essentially used as a means to  assess the compliance  of the discovered model w.r.t. given formally encoded properties. 
In~\cite{DBLP:conf/bpm/CasaluceBCV22} a so-called \emph{white-box} SMC approach is proposed by means of which traces simulated through an SMC engine are fed in to a PM framework so to yield  \emph{ model refinement}, that is to use the \emph{replayed} discovered model as a refinement of the original one. 


\vskip 2ex
    Not many methods have been proposed so far in the literature to discover  stochastic models from an event log. In Rogge-Solti \emph{et al.}'s seminal work  ~\cite{5f0e8dd04572478fb450eefe4211d69f} authors introduced a framework to discover generalised stochastic Petri net (GSPN) models extended with generally distributed timed transitions so to allow for performance analysis of the mined process. 

     Burke \emph{et al.}'s~\cite{DBLP:conf/icpm/BurkeLW20} instead address the problem of  converting a workflow Petri net, mined through a conventional  discovery algorithm, into an adequate stochastic workflow Petri net through  weight estimation. Notice that, differently from ~\cite{5f0e8dd04572478fb450eefe4211d69f}, the class of stochastic Petri net considered in this case is the subclass of GSPN whose transitions are solely \emph{immediate}, i.e., time delays are not captured by the model (hence the timestamps of the event log are ignored), only the probability of events is accounted for.   
     Specifically \cite{DBLP:conf/icpm/BurkeLW20} introduced six  weight estimators, that combine summary statistics computed on the log (e.g.,  number of times  a subsequence of activities  is observed on  the log's  traces) with statistics computed on the model and taking into account  structural relationships between the Petri net nodes (e.g.,  \emph{transitions causality}). 
     These estimators enjoy being computationally light, as, by definition, they do not need assessing the language of the Petri net model. However, the price for such simplicity is paid in terms of conformance as the distance between the resulting model's and the log's stochastic languages appears, in many cases, to be far from optimal. 
     In a follow up work~\cite{DBLP:conf/apn/BurkeLW21} the same authors introduced a framework to directly discover an \emph{untimed} GSPN model from a log based on traces' frequency. 
     
%There exist two complementary approaches to mining of stochastic models from event logs enriched with traces' frequency information. 



%Mining of stochastic models from event logs enriched with traces' frequency information can be achieved either \emph{indirectly}, i.e., without exploiting the trace frequency information in the model's mining phase,  or \emph{directly}, i.e., by devising a stochastic model straight from the frequency data contained in the event log. Indirect approaches work in two phases: first they  mine a non-probabilistic model (by application  of classical process mining algorithms) that capture  control-flow aspects of the observed process, then ``translate'' the mined model into a stochastic aimed at capturing the probabilistic behaviour exhibited in the log. 


%Stochastic process discovering via estimators~\cite{DBLP:conf/icpm/BurkeLW20}, discovering stochastic process models via \emph{toothpaste miner}, an adaptation of (inductive) miner approach~\cite{DBLP:conf/apn/BurkeLW21}, Stochastic process discovery arbitrary delay's distributions~\cite{5f0e8dd04572478fb450eefe4211d69f}

%Another relevant research aspect concerns assessing  the resemblance between stochastic languages, i.e.,  \emph{stochastic conformance checking}.  The Earth Mover Stochastic Conformance (EMSC) measure~\cite{10.1007/978-3-030-26643-1_8,LEEMANS2021101724}, relies on the adaptation of the Earth Movers Distance (EMD or Wasserstein distance) and is arguably the most  popular stochastic conformance measure however it suffers from implementation issues when it comes with applying it to languages that contain infinite words (a typical situations with models comprising loops). An alternative to EMD  is  that of \emph{entropy} related conformance~\cite{Polyvyanyy2020AnER} Most recent developments~\cite{Leemans:955905} introduced novel entropy related conformance measures based on translation of both the log and the mined model into  stochastic deterministic finite automata. 

